Hierarchical Representations for Spatio-Temporal Visual Attention Modeling and Understanding

This PhD. Thesis concerns the study and development of hierarchical representations for spatio-temporal visual attention modeling and understanding in video sequences. More specifically, we propose two computational models for visual attention. First, we present a generative probabilistic model for context-aware visual attention modeling and understanding. Secondly, we develop a deep network architecture for visual attention modeling, which first estimates top-down spatio-temporal visual attention, and ultimately serves for modeling attention in the temporal domain.

==> CHANGES <==
Changes in version 4.4 (October 2017)
o Minor clean-up, also of .gitignore 
 (thanks to Jörn Hees)
o \marginpar improved (thanks to Jörn Hees)
o Workaround for removong headlines in "list of *" 
  environments (Contents.tex and ClassicThesis.tex)
o Bibliography section headers now correctly using 
  spacedlowsmallcaps with biblatex (thanks to Ivo 
	and Enrico Gregorio)
o Added some more books to bibliography for testing
o Added help for external TikZ/PGF usage in 
  classicthesis-config.tex (thanks to Andreas Nautsch)
o Fixed redefining \marginpar for two arguments (Ivo)
o Fixed some spacing definitions and using the
  soulutf8 package now (Ivo)
o Reimplementation of \chapter and \part using solely
  titlesec and tocloft (Ivo)
o \ctparttext logic fixed (Ivo)
o Logic for detecting PDF engines, pdftex, xetex,
  luatex (Ivo)
o Support for fontspec and OpenType fonts for suitable
  PDF engines (Ivo)
o Using kvoptions package so option=value is
  available in classichtesis.sty (Ivo)
o Support for more paper sizes, fixes for headinclude
  and footinclude (Ivo)
o Fixed use of subfigure (Ivo)
o Fixed use of scrlayer-scrpage (Ivo)
o Updated the documentation (Chapter01.tex)
o Removed fixltx2e from classicthesis-config.tex and
  inserted latexrelease there and classicthesis.sty
o Added clarifications regarding use of GPL
  (ClassicThesis.tex, Chapter01.tex)

Changes in version 4.3 (not released)
o When redefining the acronym label, check for the
  acronym package's version (thanks to Scott Lowe)
o Several minor fixes (comments, whitespaces removed,
  .gitignore, .editorconfig, etc.; thanks to Jörn
  Hees)
o Updated comments regarding hyperref's draft option
  (thanks to Claudio Diaspero)
o Silenced the warnings from KOMA and titlesec about
  each other, also in the examples (thanks to Jörg
  Weber)

Changes in version 4.2 (September 2015)
o Fixed issue between titlesec and tocloft regarding
  part numbering in the ToC (classicthesis.sty).
  Thanks to Enrico Gregorio and Henri Menke.
o Fixed bug with colored lines and graffiti
  (classicthesis.sty). Thanks to Enrico Gregorio and
  Stefano Bragaglia for the fix! (Also switched
  graffiti from \slshape to \itshape.)
o Changed \vspace*{8ex} to \vspace{8ex} (Contents.tex)
o Moved \cleardoublepage from end of Contents.tex
  to appropriate position in ClassicThesis.tex
o \bflabel of acronym package removed, as it was
  removed from acronym package and caused errors.
  Now set \aclabelfont to \acsfont for consistency.
o Converted major files to UTF-8 (thanks to Jörn Hees)
  (Bibliography.bib excluded for now as BibTeX cannot
  handle UTF-8)
o Added support for BibLaTeX in
  classicthesis-config.tex and Bibliography.tex
  (thanks to Jörn Hees).
  For LyX we will have a work-around for testing.
o Added an example for one's own publication list
  (via BibLaTeX) in Publications.tex (renamed from
  Publication.tex)
o Replaced/updated scrpage2 with scrlayer-scrpage
  in classicthesis.sty (thanks to Ivo Pletìkosić).
X Worked on Appendix case with floatperchapter
  (works for captions but not for references so far)
  Thanks to Claus Lahiri and Clemens Niederberger
  for their help on this.
  [REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]
X Removed fixltx2e from classicthesis-config.tex and
  have classicthesis.sty use or emulate the latest
  LaTeX kernel via latexrelease (option: latest)
  (thanks to Jörn Hees).
  [REMOVED AS IT IS NOT AVAILABLE IN MANY
  DISTRIBUTIONS, SEE ISSUE #107]

Changes in version 4.1 (August 2012)
o Working towards XeLaTeX support:
  - "ifxetex" package for checking whether
    XeTeX is in use (classicthesis.sty)
  - Adjusted part, chapter, and tocEntry
  - Thanks to Joerg Weber for his ideas and code
  - Option "pdfspacing" does not work for XeTeX
    and is disabled when XeTeX is running
    (maybe implement spacing with fontspec later)
o Load additional packages in order to
  reduce warnings (classicthesis-config.tex)
  - "textcomp" to fix warnings with missing font
    shapes
  - "scrhack" to fix warnings when using KOMA
    with listings package
o Replaced \mathrm-command with \textrm-command
  (Chapter03.tex)

Changes in version 4.0 (December 2011)
o Due to lots of issues and complaints,
  classicthesis-preamble.sty is replaced by
  classicthesis-config.tex (which is cleaner,
  nicer, better, etc. than before!)
o No per-chapter-numbering also for equations
  (classicthesis.sty and Chapter03.tex)
o classicthesis.sty now also works without the
  KOMA-classes (scrbook, scrartcl, etc.):
  - This affects the text body shape, where the
    package "typearea" is always loaded in order
    to use \areaset
  - And affects the layout of footnotes where the
    package "footmisc" is loaded otherwise
    (not 100\% identical look-and-feel but OK)
o Help for using spanish babel with classicthesis
  (classicthesis-config.tex)
o Note about pdfsync issues with graffiti
  (Chapter01.tex)
o Minor clean-up of comments and duplicate lines
  (classicthesis.sty)
o Adjusted the colophon text (Colophon.tex)
o Increased space for labels in the LoF, LoT, LoL
o Included version information on the title page and
  in the drafting and final version information
  (classicthesis.sty and Titlepage.tex)

Changes in version 3.0 (June 2011)
o There have been some major changes in order to port
  classicthesis to LyX easily. See below for details.
  Special thanks go to Ivo Pletikosi\'c for all his
  hard work he put into this project!
o Changes in ClassicThesis.tex:
  - Redundant fleqn removed from documentclass options
   (will be set by amsmath package in preamble)
  - KOMA adjustments for documentclass:
    fontsize=11pt,paper=14
  - Moved language options into documentclass due to LyX
    issues with babel
o Changes in classicthesis.sty:
  - Removed bcor from \areaset command so that it can
    be set via \documentclass option (BCOR=)
  - New \ctparttext command for putting preamble text
    after part titles (see ClassicThesis.tex for examples)
  - \graffito command now also available as original
    \marginpar (backward compatibility is enabled)
  - Chapter number in margin done with \oldmarginpar
o Changes to classicthesis-preamble.sty:
  - Fixed autoref for subfigures (see Chapter 2 for example)
  - Fixed issues with redefining autoref strings (for
      different languages)
  - Now contains all configuration information, such as
    the title, your name etc.
  - This package now also loads classicthesis.sty, change
    the options classicthesis to be loaded with here
  - Package inputenc now loaded with latin9 option
  - Package listings now also loaded here
  - Now safer package loading regarding options by
    using \PassOptionsToPackage command extensively
  - Inserted new string for \mySubtitle
o Changes in Titlepage.tex and Titleback.tex because of new
  string \mySubtitle
o Changed a lot of the documentation, e.g., in Chapter01.tex

Changes in version 2.9 (January 2011)
o Fixed onlytext euler font for MinionPro font (in
  classicthesis.sty)
o Option "listsseparated" deprecated, because it led to some
  strange side-effects (in classicthesis.sty)
o Changed default font size to 11pt (in ClassicThesis.tex) and
  adjusted text block size accordingly (in classicthesis.sty)
o Fixed bug with backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o New option "floatperchapter" for classicthesis.sty, removed
  all code for that from classicthesis-ldpkg.sty
o Removed "nochapters" option from classicthesis-ldpkg.sty
o Removed redundant loading of listings package (in
  classicthesis-ldpkg.sty)
o Fixed some headline bug in example classicthesis-book.tex
o Fixed a bug when using parts with plain latex as in example
  classicthesis-book.tex (in classicthesis.sty)

Changes in version 2.8 (March/May 2010)
o Fixed serious \graffito bug in classicthesis.sty
  (thanks to Lorenzo Pantieri and Enrico Gregorio)
o Included backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o Fixed drafting issues (draft information not shown at all)
  caused by wrong code for listings and listsseparated options
  in classicthesis.sty

Changes in version 2.7 (February 2010, cumulative release)
o Removed option for classicthesis-ldpkg.sty: nobackref
  Introduced instead option "backref" for consistency
  which works the other way (no backrefs by default)

Changes in version 2.6.2 (January 2010, released as beta)
o New option for classicthesis-ldpkg.sty: nobackref
  (removes links to cited page in bibliography)
o Fixed some spacing issues for LoF, LoT, LoL with option
  "listsseparated" (in classicthesis.sty)

Changes in version 2.6.1 (October 2009, released as beta)
o Removed \myChapter and \myPart, you can now use the regular
  \chapter and \part commands (in classicthesis.sty)
  (thanks to Hinrich Harms for this)
o Fixed used KOMA-options: numbers=noenddot, cleardoublepage=empty
  (in ClassicThesis.tex)
o Included hack to use citations in float environments, will
  be fixed with caption package version 3.2 (in classicthesis.sty)
o Included some font and text area fine-tuning code
  (in ClassicThesis.tex)
o Some testing with Libertine font (classicthesis-book.tex)
o Fixed numbering of listings used in different chapters
  (in ClassicThesis.tex, classicthesis.sty, classicthesis-ldpkg.sty)
o Spacing between listings in different chapters and after List
  of Listings header fixed (in classicthesis.sty)
o Increased \newnumberwidth to sizeof(999) which is better for
  documents with more than 99 pages (in classicthesis.sty)
o New option for classicthesis.sty: manychapters

Changes in version 2.6 (August 2009)
o Centered the title page with the addmargin environment
  (thanks to Nicolas Repp for the hint)
o Fixed header for page two of Table of Contents (with 3
  or more pages) (in Contents.tex)
o Added numbering of \subsubsection (in Contents.tex)
o Added correct Table of Contents entries for \subsubsection
  (in classicthesis.sty)
o Added printonlyused option to loading acronym package
  (in classicthesis-ldpkg.sty)
o Some code for "clean" hyperlinks (w/o color and w/o boxes)
o Minor fix for \graffito (in classicthesis.sty)

Changes in version 2.5.1 (May 2009, released as beta)
o New option for classicthesis.sty: dottedtoc
  (Refer to the manual for more information.)
o New option for classicthesis.sty: listings
  (Refer to the manual for more information.)
  (Credit + thanks to Prof. Enrico Gregorio)
o Minor clean-up and bug-fixing

Changes in version 2.5 (October 2008, cumulative release)
o Increased text-width for better page layout (experimental)
o Cumulative release, some minor clean-up and bug-fixing

Changes in version 2.4.{1--3} (February and April 2008,
released as betas)
o Switched back to "obsolete" KOMA options due to
  compatibility issues on some installations
o Increased robustness of \cauthor command in
  classicthesis-ldpk.sty
o Spacing fix for \sectionmark (in classicthesis.sty)
o Made Booleans private (in classicthesis.sty)
o Acronyms header for long acronym lists (in Contents.tex)
o Moved "amsmath" package from classicthesis.sty to
  ClassicThesis.tex
o "MinionPro" package now loaded with "mathlf" option
  instead of "osf" option (in classicthesis.sty)
o Fixed issue with contents headings (in classicthesis.sty
  and in Contents.tex)
o Thanks to Lorenzo

Changes in version 2.3 (November 2007)
o Fixed serious bug with \myChapter command (using plain
  LaTeX)
o Removed hypcap package from classicthesis-ldpkg.sty and
  placeins package from classicthesis.sty. Put both into
  ClassicThesis.tex for finer end-user control
o Removed obsolete KOMA options from ClassicThesis.tex
o Option "subfigure" deprecated, replaced by "subfig" (in
  classicthesis.sty)
o Inserted some mechanisms to detect whether subfig(ure)
  package was loaded or not (in classicthesis.sty)
o Inserted some mechanism to detect whether classicthesis
  packackage was loaded or not (in classicthesis-ldpkg.sty)
o Moved "headlines" code block a bit up in
  classicthesis.sty (seemed to cause problems with new
  KOMA-Script classes)
o Removed accidental "natbib" from classicthesis-ldpkg.sty
o Some fine-tuning in (Dirty)Titlepage.tex
o Thanks to Lorenzo and Denis! :-)

Changes in version 2.2 (October 2007)
o \myChapter and \myPart now take an optional argument
  just as the regular \part and \chapter commands
o Did some minor changes to classicthesis-book.tex
  so it's a better example
o Inserted some \cleardoublepage before \myPart
  occurences to avoid pdfbookmark problems
o Introduced some general typographic fine-tuning
  (linespread, penalties, etc.)
o Did some fine-tuning of the \graffito command

Changes in version 2.1 (July 2007)
o Removed duplicate xcolor package call from
  classicthesis-ldpkg.sty and shifed some color
  definitions around
o Removed re-definition of \ttdefault

Changes in version 2.0 (June 2007, cumulative release)
o Better setup of the list of acronyms
  (in classicthesis-ldpkg.sty)
o Using KOMA option footinclude in ClassicThesis.tex
  (text block sizes are adjusted to this)
o New option for classicthesis.sty: minionpro
o New option for classicthesis.sty: minionprospacing
o New option for classicthesis.sty: pdfspacing
  (Refer to the manual for more information.)

Changes in version 1.7 (May 2007, not released separately)
o Removed \graphicspath from ClassicThesis.tex
o Use the nag package to ensure "compliance"
o Switched from ccaption to caption in classicthesis-ldpkg.sty
  (setup via \captionsetup in ClassicThesis.tex)
o Switched from subfigure to subfig in classicthesis-ldpkg.sty
o Removed obsolete "usenames" option from loading xcolor package
o Noticed problem with \thelstlisting on some installations
  (commented out in classicthesis-ldpkg.sty)
o Noticed problem with some hyperlinks on some installations
  (could not determine cause)

Changes in version 1.6 (April 2007, not released separately)
o Included greetings to Lorenzo Pantieri for many very useful
  suggestions
o Introduced new commands in classicthesis-ldpkg.sty to make
  adaptation of backrefs to different languages easier
   - \backrefnotcitedstring (ref is not cited)
   - \backrefcitedsinglestring (ref is cited on one page)
   - \backrefcitedmultistring (ref is cited on multiple pages)
o Removed ellipsis package from classicthesis-ldpkg.sty due to
  some undesired results for some users
o Removed the following packages from classicthesis-ldpkg.sty as
  these seem to require changes to their options from most users:
  inputenc, babel, natbib (now in ClassicThesis.tex)
o New option for classicthesis-ldpkg.sty: nochapters
  Use the package with classes that do not have chapter divisions

Changes in version 1.5 (April 2007, not released separately)
o Fixed some bugs to use classicthesis.sty for article layout
o Inserted some info/warnings when using nochapter/parts
o Extended the manual: examples for using classicthesis.sty for
  other projects than a thesis (source available in folder
  "Examples")
o Some minor adjustments in classicthesis-ldpkg.sty
o Fixed some spelling mistakes

Changes in version 1.4.2 (March 2007)
o Renamed loadpackages.sty to classicthesis-ldpkg.sty due to
  TeX Live package tree issues

Changes in version 1.4.1 (March 2007)
o Fixed some wording concerning the license :-o
o Added fixltx2e and ellipsis packages to to loadpackages.sty to correct
  some minor glitches
o Fixed and changed some things about ToC entries of parts
o Some minor bug fixes

Changes in version 1.4 (January 2007)
o Replaced \lineheight with \baselineskip in classicthesis.sty
o Removed obsolete "usenames" option from xcolor package (classicthesis.sty)
o Now classicthesis.sty processes the global a5paper option and adjusts
  the layout accordingly (experimental!)

Changes in version 1.3.1 (August 2006)
o Urgent bug concerning ToC spacing etc. fixed

Changes in version 1.3 (August 2006)
o New option for classicthesis.sty: parts
  Turn this on if you use Part divisions. It fine-tunes the ToC and
  adds support for Part division via \myPart{} (cf. \myChapter{})
  (The style of this feature is preliminary, any suggestions?!)
o New option for classicthesis.sty: eulermath
  Uses the awesome Euler fonts for math (Palatino fonts are default).
o Added mparhack package to loadpackages.sty to get the graffiti right
o Added a hint to loadpackages.sty on how to typeset the List of
  Listings consistently with classicthesis
o Some minor fine-tuning of typographic details
o Collaboration with babel package improved (now easier to use
  with other languages than English)
o Added appropriate textwidth values for 11pt Palatino and Minion
  (See comments near \areaset in classicthesis.sty)
o Note: There is a problem with the case of math text in part-,
  chapter-, and section titles and I have no clue how to fix this
  (either the case or the spacing breaks). So far, I chose the case. :-(

Changes in version 1.2 (June 2006)
o Setup a little postcard collection: http://postcards.miede.de
o Changed stupid spelling mistake: "A Homage" => "An Homage" D'oh!
o New option for classicthesis.sty: nochapters
  Allows to use the look-and-feel with classes that do not use chapters.
o New option for classicthesis.sty: beramono
  Loads Bera Mono as typewriter font. (Default = no typewriter font.)
o Included list of files, see LISTOFFILES.

Changes in version 1.1 (May 2006)
o classicthesis.sty now stand-alone and usable w/o whole bundle!
o classicthesis.sty compatible with both LaTeX and PDFLaTeX
  Note: this is only true for classicthesis.sty, not the whole bundle.
o New option for classicthesis.sty: subfigure
  Tells the style to add the respective option when loading tocloft.
o Now loading microtype package w/o options (classicthesis.sty)
o Fixed overfull hbox warnings for ToC entries (classicthesis.sty)
o No longer depending on a particular caption package (classicthesis.sty)
o Layout for subsubsections provided (classicthesis.sty)
o PDF opens on title page (ClassicThesis.[tex|pdf])
o Files are a bit more "ASCII-friendly" (all)
o Note: Thanks to all the folks who already sent me a postcard! :-)

Version 1.0 (March 2006)
o First public release


==> Chapters/Chapter01demo.tex <==
%************************************************
\chapter{Introduction Demo}\label{ch:introduction_demo}
%************************************************
This bundle for \LaTeX\ has two goals:
\begin{enumerate}
    \item PhD thesis.
    \item ``\emph{The Elements of
    Typographic Style}'' \citep{bringhurst:2002}.
    \marginpar{\myTitle \myVersion}
\end{enumerate}

If you like the style then I would appreciate a postcard:
\begin{center}
    André Miede \\
    Detmolder Straße 32 \\
    31737 Rinteln \\
    Germany
\end{center}
The postcards I received so far are available at:
\begin{center}
    \url{http://postcards.miede.de}
\end{center}

\paragraph{Important Note:} Some things of this style might look
unusual at first glance, 
\begin{itemize}
    \item See the documentation for the \texttt{booktabs} package for
    a nice discussion of this topic.\footnote{To be found online at
    \url{http://mirror.ctan.org/macros/latex/contrib/booktabs/}.}
    \item And last but not least,
\end{itemize}

\paragraph{Yet Another Important Note:} Since \texttt{classicthesis}'
first release in 2006
\graffito{An outlook into the future of \texttt{classicthesis}.}

\section{Organization}


\clearpage
\section{Style Options}\label{sec:options}
There are a couple of options for \texttt{classicthesis.sty} that
allow for a bit of freedom concerning the layout:
\marginpar{\dots or your supervisor might use the margins for some
    comments of her own while reading.}
\begin{itemize}
    \item General:
        \begin{itemize}
            \item\texttt{drafting}: prints the date and time at the bottom of
            each page, so you always know which version you are dealing with.
            Might come in handy not to give your Prof. that old draft.
        \end{itemize}
\end{itemize}

\section{Customization}\label{sec:custom}
%(As of v3.0, the Classic Thesis Style for \LaTeX{} and \mLyX{} share
%the same two \texttt{.sty} files.)
\begin{lstlisting}
    % **************************************************
    % 2. Personal data and user ad-hoc commands
    % **************************************************
    \newcommand{\myTitle}{A Classic Thesis Style\xspace}
    \newcommand{\mySubtitle}{An Homage to...\xspace}
\end{lstlisting}

%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/Chapter02.past.tex <==
%*****************************************
\chapter{A multidisciplinary perspective on visual attention}\label{ch:visual_attention}
%*****************************************

\section{Introduction}\label{sec:introduction_2}
%SIMONE FRINTOP
%Computational Visual Attention Systems and their Cognitive Foundations: A Survey
%- World
%- Eye: Information capture. Fixations mechanism.
%- Brain: Attention is the process by which the brain controls and tunes information processing.
%- Image
%https://www.ics.uci.edu/~majumder/vispercep/vispercepold.htm
%PIZLO Course
%Palmer, 1999
During the 1970s, scientists from several disciplines began to show a great interest in understanding how optical images could be processed to extract useful information about the environment. This resulted in the emergence of vision science. 

Vision science \cite{Palmer} is defined as an interdisciplinary branch from cognitive science which is devoted to the study of visual mental states and processes from different, compatible and complementary perspectives. All of them talk about vision in the common language of computation, by accepting that it may take place not only in living organisms, through eyes and brains, but also when information from cameras is processed in ad-hoc programmed computer systems.  

Over the past few decades, psychologists have tried to explain visual perception through a vast amount of theories and models. On the other hand, neurophysiologists have made experiments to monitor neuron activity. Moreover, computational neuroscientists have built neural network architectures to simulate how these neurons represent and react to visual stimuli. Drawing on these findings, computer vision scientists have sought to develop computational models and algorithms which automatically address the cognitive functions involved in attention. 
  
Indeed, a great world full of visible information is opened to us, and the \acf{HVS} has the paramount task of dealing with attentive processes. Due to the limited capacity of the brain to process such a big amount of sensory input, attention involves the inherent search operations that reformulate and optimize generic perception and cognition problems so that they become tractable \cite{TsotsosBook}. Eye movements allow acquiring and tracking visual stimuli, unconsciously highlighting the most conspicuous \cite{BruceT05} \cite{Itti_Baldi06nips} areas in a particular context, or willingly selecting those that aid to solve a particular task \cite{sprague2003eye}. 

This thesis presents a framework for visual attention estimation and understanding from a computational view, not only applying existing computer vision techniques, but also contemplating psychological arguments and neurological structures. This chapter makes a review of the most relevant and recent related work in perception and visual attention, bearing in mind all the perspectives differentiated above. The purpose of this \emph{state-of-the-art} is thus to provide a broad overview of the visual attention research by identifying the basis of our work.
 
\section*{Chapter overview}
Starting from the structure and the processes involved in the eyes and the brain, visual attention is reviewed from a neurophysiological perspective in Section \ref{sec:neuro_va}. We discuss the difference between overt attention, which implies eye movements and fixations, and covert attention, which is more related to the mechanisms of the brain for visual selection and representation. Then, Section \ref{sec:psy_va} introduces the most outstanding psychological theories of visual attention, which allude to \emph{early representation} features that guide the attention of observers. Moreover, we also cover some noticeable studies on the the role of eye movements. Finally, we summarize some of the existing computational models of visual attention in Section \ref{sec:computational_va}, mainly attending to those approaches close to the contributions of the thesis.

\section{Neurophysiological basis of visual attention}\label{sec:neuro_va}
This section describes the structure of the \acs{HVS}, attending to the regions of the eye and the nervous system that take part in the process of visual perception. According to \cite{Palmer}, visual perception is an information extraction process that involves the acquisition of knowledge about objects and events in the environment. This information comes from the light that is emitted or reflected by objects. 

It should be noted that \acs{HVS} has an extraordinary ability to select only the necessary information in order to interact with a given scenario, being able to infer the rest with sufficient accuracy. Hence, given an image, vision implies a heuristic process to infer the most likely environmental condition that could have produced it. 
  
\subsection{Human Visual System: eye and brain}\label{sec:neuro_va1}
Both eyes and brain are essential for visual perception. The complete eye-brain system must perform adequately to obtain trustworthy visual data. 

\begin{figure*}[!t]
\centering
    \includegraphics[width=1\textwidth]{gfx/chapter2/221_human_eye2.eps} %\quad
    \caption[Diagram of the human eye.]{Diagram of the human eye. Rods and cones densities are drawn around the retina in blue and red, respectively. Adapted from Wikimedia Commons \cite{human_eye_diagram}.}
    \label{fig:hvs_eye}
\end{figure*}

\subsubsection*{The eye} 
The structure of the human eye is shown in Figure \ref{fig:hvs_eye}. Humans have two approximately spherical eyes. They are situated at two holes in the skull called \emph{eye sockets}, which are placed at about the horizontal midline of the head. Eyes are moved by six small and strong \emph{extraocular muscles}, which are responsible for eye movements, allowing to scan different regions of the visual field. They are monitored by several nuclei in the brain stem, via the oculomotor neurons.

Several parts of the eye carry out optical functions. First, eyes collect information in light that enters through the \emph{cornea}. The light crosses an opening in the \emph{iris} called \emph{pupil}, behind which the \emph{lens} is located. Finally, incoming light projects an image onto the \emph{retina}, a curved surface at the back of the eye. The retina is composed of more than 100 million light-sensitive cells, known as \emph{photoreceptors}, which transform light into neural activity. There are two types of photoreceptors: rods and cones. As can be seen in Figure \ref{fig:hvs_eye}, rods, which are long and numerous (about 120 million), are located everywhere in the retina except at its center. They are highly sensitive to light, so they allow us to see at low light levels or \emph{scotopic conditions}. In contrast, most of the cones, which are shorter and fewer (8 million), are clustered in the \emph{fovea}, situated at the center of the retina. They are much less sensitive to light, used under normal lighting or \emph{photopic conditions}, and also in all experiences of color.

Light comprises photons, many small units of energy that produce electrical changes in photoreceptors, and the information travels via the \emph{optic nerves} to the visual centers in the brain. 

\subsubsection*{The brain}\label{sec:brain}
\begin{figure*}[!t]
\centering
	\includegraphics[trim=0cm 0cm 0cm 0cm, width=0.9\textwidth]{gfx/chapter2/221_neuron.eps}	
\caption[Schematic diagram of a biological neuron.]{Schematic diagram of a biological neuron. Adapted from \cite{Palmer,cs231n}.}
\label{fig:221_neuron}
% \vspace{-0.4cm}
\end{figure*}
From the fovea in each eye, the optic nerves cross over to the opposite side of the brain, leading the information from the left half of the visual field to the right side of the brain and vice versa. The brain processes this information, in order to make it useful for observers.

\emph{Neurons} constitute the basic computational cells of the brain. The human brain is composed of around 100 billion neurons. As shown in Figure \ref{fig:221_neuron}, a neuron first receives electrical signals coming from other neurons across the \emph{dendrites}, such as photoreceptors in \acs{HVS}. Within the \emph{cell body}, where the \emph{nucleus} is located, these inputs are converted then into a series of output spikes that are propagated through its \emph{axon} to other neurons. The \emph{firing rate} of the neuron determines the frequency of the spikes. Finally, \emph{synapses} connect the axon to the dendrites of the following neurons.   

There are two pathways on each half of the brain. One of them arrives to the \acf{SC}, which seems to be involved in the control of eye movements by processing information related to the location of objects in the world; the second and larger pathway goes to the \emph{occipital} or \acf{V1}.

Nowadays, we have an evidence about the function of the \emph{occipital}, \emph{parietal} and \emph{temporal lobes} of the visual cortex, which are identified in Figure \ref{fig:221_brain}. The cortical processing begins at \acs{V1} cells, where spatial \emph{receptive fields} respond to visual stimuli, so that a mapping of the information from the retina is produced. According to the scale-space theory of computer vision \cite{lindeberg2013computational}, receptive fields encode simple visual patterns of light, such as oriented edges or color blotches, which constitute the first stages of visual processing, by reflecting the symmetry properties of the world that surrounds us. Moreover, a reduced set of operations over these simple patterns allow to obtain a wide variety of complex underlying representations for visual perception. \acfp{CNN} \cite{lecun1989backpropagation} emerged in an attempt to reproduce the function of receptive fields, recently demonstrating an astonishing performance in a lot of applications. They will be described in section \ref{sec:convolutional_neural_networks}, as the basis of our contributions for visual attention estimation in the temporal domain in Chapter \ref{ch:anomaly_detection}.

The information from \acs{V1} is then projected to other parts of the occipital lobe, and also to areas of the parietal and temporal ones. Some studies \cite{zeki1978functional, livingstone1988segregation} suggest that these different regions involve small maps where several properties derived from the retinal stimulation are coded in parallel, such as color, form, depth and motion. Regarding the parietal and temporal cortex, they seem to be responsible for the identification and location of objects, respectively. 

\begin{figure*}[!t]
\centering
	\includegraphics[trim=0cm 0cm 0cm 0cm, width=1\textwidth]{gfx/chapter2/221_brain.eps}	
\caption[Diagram of the human brain.]{Diagram of the human brain. Arrows indicate the connection between the eye and the principal areas in the brain involved in the visual attention process: frontal eye fields and posterior parietal cortex, which guide spatial attention, and the \acf{SC}, which controls both eye movements and covert shifts of attention. Eye and brain diagrams taken from Wikimedia Commons \cite{human_eye_diagram, brain_diagram}.}
\label{fig:221_brain}
% \vspace{-0.4cm}
\end{figure*}

\subsection{Visual attention}\label{sec:neuro_va2}
%YARBUS
%Eye movements (See journal article), visual attention
Visual perception is inherently selective \cite{Palmer}. We are able either to globally process the information in a scene, or to focus our vision more on some particular objects.
We sometimes even attend locally to their specific parts or properties, depending on their importance in the activity we are performing. In addition, we choose quite automatically where to fixate our vision next. For instance, although there may be a lot of appliances in a kitchen, we immediately head towards the fridge if we want to drink something, without looking at the toaster or the dishwasher. %In the same way, if we are going to cook a pizza, we barely have to think about going from the fridge, where we will first take it, to the oven. 

All these strategies for selecting and processing information in the visual field are related to attention. Two different acts of visual attention can be distinguished. First, attention is called \emph{overt} if it is external and observable by others, implying eye movements to fixate from one object to another. Different fixations of a context contain useful information which is shaped like visual images on the retina. Then, part of the fixated information is selected by \emph{covert} attention to be fully processed. Covert selections are, conversely, internal and unobservable by others. They do not imply eye movements, but allow to shift our gaze to peripheral Regions Of Interest (\acsp{ROI}), chosen from the information processed.

\subsubsection*{Overt attention: eye movements and fixations} 
Visual attention can be thus described, on the one hand, as a temporal process that involves a sequence of eye fixations preceded by different types of eye movements. This results in a series of instantaneous spatial locations of the visual axis called \emph{gaze points}.

There are four basic types of \emph{eye movements} \cite{purves2001neuroscience}. If we look at still images or static objects, we mainly perform saccadic movements to scan over them. \emph{Saccades} are very quick (20-40 ms) voluntarily or involuntarily ballistic jumps between two points of fixation. During a saccade, both eyes drift in the same direction. Moreover, the trajectory of a saccade cannot be changed when the eyes are in motion.

In real-life situations, where either the viewer or the objects are moving, three more types of eye movements can be found:

\begin{itemize}

\item \emph{Smooth pursuit movements}, which are slow in comparison with saccades, are used to track the position of moving objects. The ability of the \acs{HVS} to take clear images from tracked objects depends on how fast they move, being less accurate at speeds higher than 30 degrees per second, when subjects start to use saccades to follow objects. 

\item \emph{Vergence movements} allow \acs{HVS} to fixate objects located at different depths. In this type of movement, eyes move in opposite directions and have an angle of convergence that depends on the distance of the target from the observer. Near objects cause strong convergence, while far objects almost result in it.  

\item \emph{Vestibular movements} are controlled by the vestibular system in the inner ear, and contribute to keep the target fixed on the fovea when the head changes its position and orientation (ego-motion). In this situation, eyes compensate the ego-motion by moving in the opposite direction of the head, normally at its same speed.

\end{itemize}

When the eyes stop examining the scene, \emph{fixations} take place and the \acs{HVS} takes comprehensive information about what is being looked at. Although it is not often mentioned, fixations are not directly measurable, but composed of minute microsaccades, tremor and drift movements that focus the eyes on the target, generating multiple gaze point samples. They have a particular duration, usually between 50-600 ms, and can reveal meaningful information about attention and understanding. Given a specific context, the time to first fixation in a conspicuous location or target is short, while a long fixation duration may suggest a greater effort to make sense of a stimulus, or an appealing one.

All these movements have disparate neural mechanisms, which are spread in different areas of the brain, as shown in Figure \ref{fig:221_brain}. First, frontal eye fields in the frontal cortex control the voluntary saccades. On the other hand, both smooth pursuit and vergence movements require visual feedback, so they are monitored by means of information from the motion channels in visual cortex and binocular disparity channels in occipital cortex, respectively. Finally, vestibular movements result from disturbances in the fluid of the semicircular canals of the inner ear. These are monitored by the vestibular system, which connects to the oculomotor neurons to provide them with the correct eye velocity signal. The \acs{SC} is also involved in the control of eye movements, as was mentioned above. 

\subsubsection*{Covert attention: Relation with overt attention}
On the other hand, \emph{visual attention} concerns a set of complex covert processes that aid an observer to select and gather the most outstanding information within the visual field, with the aim of successfully solving a cognitive problem in a particular environment.

Covert attention is usually directed at the \acs{ROI} fixated by the eyes. Stephen E. Palmer \cite{Palmer} makes an interesting metaphor in order to explain the relationship between eye movements and covert attention: \emph{"Attention is like an internal eye that can be moved around to sample the visual field much as the eye can be moved around to sample the visual world."} What is more, there is evidence that eye movements usually follow attentional movements. Thus, covert attention, viewed as the primary function of visual selection, controls overt saccades, which play an important but supporting role, driving them to the appropriate locations and enhancing the perception of events happening there. 

Therefore, it is known that there exist a strong correlation between the areas in the brain that controls eye movements and covert attention: \acs{SC} controls both eye movements and covert shifts of attention, while frontal eye fields and the posterior parietal cortex are responsible for guiding spatial attention. Arrows in Figure \ref{fig:221_brain} indicate the connection between the eye and the principal areas in the brain involved in the visual attention process.

Finally, many studies agree in saying that this frontoparietal network may involve an attentional \emph{priority map} \cite{bisley2011neural}, which represents items in the visual world according to their importance in a particular situation. We will discuss more about the utility of this representation of visual attention in the next section, now from a psychophysical perspective.

\section{Psychophysical theories of visual attention}\label{sec:psy_va}
%TREISMAN AND GELADE, WOLFE...
%Psychological Basis of Visual Attention
%(See journal article)
In this section, we gather the statements of the most outstanding psychological theories of visual attention, which establish relevant features for the perception of objects and support the majority of existing computational attention systems \cite{frintrop2010computational}. 

Two fundamental theories have been the most influential: the \acf{FIT} \cite{TreismanGelade80} and the \acf{GSM} \cite{wolfe1994guided}. Based on the foundations of these studies, we can differentiate between two main families of visual attention models: \acf{BU} or \emph{stimulus-driven} and \acf{TD} or \emph{task-oriented}. In addition, it is also worth mentioning the importance of eye movements in scene perception, as explained in the famous classic study of Yarbus \cite{Yarbus1967}. 

In addition, we refer for the first time to several aspects that have been considered in the design of the probabilistic model for visual attention understanding presented in Chapter \ref{ch:atom}.

\begin{figure*}[!t]
\centering
	\includegraphics[trim=0cm 0cm 0cm 0cm, width=1\textwidth]{gfx/chapter2/23_psycho_theories.png}	
\caption[Diagram representations of (a) the \acf{FIT} and (b) the \acf{GSM} \cite{wolfe1994guided}.]{Diagram representations of (a) the \acf{FIT} \cite{TreismanGelade80}, where visual attention is modeled as a combination of intensity, color and orientation pre-attentive features, and (b) the \acf{GSM} \cite{wolfe1994guided}, which introduces ``guiding representation'' as a control mechanism before object recognition, and also mentions new features such as size, motion or depth. Adapted from \cite{WolfeHorowitz04}. Eye diagrams taken from Wikimedia Commons \cite{human_eye_diagram}.}
\label{fig:23_psycho_theories}
% \vspace{-0.4cm}
\end{figure*}

\subsection{The Feature Integration Theory}
Treisman and Gelade introduced the \acf{FIT} \cite{TreismanGelade80} in 1980, which states that several features or attributes are identified early, automatically and in parallel across the visual field, while objects are registered separately as a conjunction of these features at a later serial stage. The model is depicted in Figure \ref{fig:23_psycho_theories}(a). A master map of location results from this combination of attributes, which indicates where the objects are, prior to their recognition.

In light of this theory, Treisman discussed the difference between feature and conjunction search processes, when looking for a target in a scenario full of distractors. In a \emph{feature} or parallel search process, we seek through distractors that differ from the target by a unique feature. In contrast, Treisman asserted that a \emph{conjunction} or serial search assumes a more complex and time-consuming task, since the distractors have one or more features in common with the target. The more attributes aid to discern the target from the distractors, the easier the search for a target is. Nevertheless, if we know the features of the target in advance, conjunction search performance can be improved by inhibiting the features which are exclusive from distractors.

% In the same way that other behavioral analysis [COMPLETECITE], \acs{FIT} mentions three basic features: intensity or luminance contrast, color and orientation.

\subsection{The Guided Search Model}
The standard \acs{FIT} defines parallel and serial search as autonomous processes that cannot share information between them. By contrast, Wolfe's \acf{GSM} 2.0 \cite{wolfe1994guided} from 1994 claims that the \acs{FIT} attentive serial search has to be guided by useful information in the preattentive parallel processes, which divided their corresponding set of stimulus into distractors and candidate targets. 

\acs{GSM} thus supports that attention can be guided towards specific targets by modulating gains associated with low-level features. Indeed, visual search is a continuous process and, consequently, the information from the parallel processes to the serial process can be updated over time.

Subsequents works by Wolfe \cite{WolfeHorowitz04} \cite{Wolfe2007guided} 
present the idea of ``guiding representation'' or guidance as a control device located to one side of the main pathway from early vision to object recognition, as shown in Figure \ref{fig:23_psycho_theories}(b). It controls the access to the attentional bottleneck, so the guidance is abstracted from the main pathway despite of not being part of the pathway itself. Thus, the way we see stimulus in the world is different from the representations upon which guidance is founded. Rather than altering the stimulus such as filters would do, this module guides attention as a CCTV operator working at a public building (e.g. a train station or a university) would do. Based on an abstract representation of some notions (e.g. threat, suspicious object), the operator selects some parts of the scenario that receive more attention than others. 

Two ways of guidance are possible, \acf{BU} and \acf{TD}, which correspond to the two main types of computational visual attention systems. \acs{BU} attention is fast, involuntary and mainly based on characteristics of the visual scene (\emph{stimulus-driven}) such as color, orientation, motion or depth. By contrast, \acs{TD} attention is slow, voluntary and determined by cognitive phenomena like knowledge, expectations or advanced indications (\emph{goal-driven}). 

Guidance can be ultimately represented as an activation map. An activation map drawn only by \acs{BU} signals is a \acf{SM} \cite{koch_shifts}. Instead, \acs{TD} guidance provides a priority or \acf{VAM} that sorts by relevance the items existing in the visual field for selective attention and recognition \cite{wolfe2014approaches}. 

It is also worth noting the concept of scene guidance incorporated in the version 4.0 of \acs{GSM} \cite{wolfe2011visual}, which results in a non-selective pathway in the visual search process: Observers are able to determine very rapidly the global properties or `gist' of a given scene (e.g. a highway with intense traffic) before they selectively attend to the most conspicuous objects (e.g. a damaged car). 
% Completar esta parte si finalmente se incorpora a alguna parte de nuestro modelo!!!

Hence, guidance is not based directly on the information provided by early visual processes but on a coarse and contextual representation derived from them. This interpretation of visual attention supports the main assumption of our model and opens the door to the inclusion of an intermediate layer mapping the low level stimuli to an intermediate representation. 
% Dejo sin explicar re-entrant process (Wolfe, Oxford Attention, Pag. 23)
% y busqueda de objetos como proceso de difusion (Pag. 36)

\subsection{What are the attributes that guide attention?}
A significant number of authors have contributed to determine a wide set of features that might drive attention, as outlined in the excellent review by Wolfe \cite[Chapter 2]{wolfe2014approaches}. In this survey, features are grouped depending on their consensual reliability, which is determined taking into account both the number of studies that support them and the convergence of their demonstrations. Some of these features are more effective than others, not only because of what they measure but also depending on the quality of the visual support where they are computed. 

First, Treisman and Gelade's \acs{FIT} \cite{TreismanGelade80} mentioned three basic features: intensity or luminance contrast, color and orientation. These are considered undoubted attributes, so they constitute the basis of almost all the existing models that explain visual attention.

Additionally, Wolfe's \acf{GSM} 2.0 \cite{wolfe1994guided} enumerated other attributes that humans can perceive efficiently and thus could be also considered salient in a scene: motion, scale or size, shape and depth. According to McLeod et al. \cite{mcleod1988visual}, motion speed and direction could be represented separately. Moreover, it is also unclear if shape should be defined as a whole or, alternatively, as a family of simpler attributes such as curvature, line termination or closure. Then, depth aid to modulate features like size. Near objects stand out from far ones, which seem to be smaller. Wolfe later extended this list \cite{WolfeHorowitz04}, raising doubtful or complicated cases such as novelty, faces or other semantic categories (e.g. `car' , `dog').  

Based on psychologists intuition, we have selected some of these attributes as input to our approach for visual attention understanding, with the purpose of appraising their utility in diverse contexts. Chapter \ref{ch:atom} introduces this set of features, as well as the image processing techniques used for their extraction.

%\begin{table}
%    \myfloatalign
%    \begin{tabularx}{\textwidth}{lll} \toprule
%        \tableheadline{Undoubted attributes} & \tableheadline{Probable attributes}
%        & \tableheadline{Complicated attributes} \\ \midrule
%        Intensity & Shape & Novelty \\
%        Color & Depth & Faces \\
%        Orientation &  & Text \\
%        Motion & & Semantic category (e.g. 'car', 'dog') \\
%        Size & & \\
%        \bottomrule
%    \end{tabularx}
%    \caption[]{Examples of attributes that might guide visual attention. Features are grouped according to their consensual realiability, which has been determined taking into account both the number of studies that support them and the convergence of their demonstrations. Table adapted from \cite{WolfeHorowitz04} \cite{wolfe2014approaches}}  \label{tab:guiding_atributes_examples}
%\end{table}

\subsection{Eye movements}
The role of eye movements in scene perception had already been studied before the introduction of the perception theories referred above. According to the revision of previous research on high-level scene perception made by J. M. Henderson and A. Hollingworth \cite{henderson1999high}, one can figure out what are the procedures that control \emph{where} and \emph{how long} each fixation point tends to remain centered at a particular location to provide a complete understanding of scene. 

Yarbus classic study of 1967 \cite{Yarbus1967} showed that, although first few fixations in a scene seem to be controlled by global characteristics, positions of later fixations are not random but landed on regions that are useful or essential for perception. Eyes are either driven by \acs{TD} factors that direct fixations toward task-driven informative locations (e.g. cooking, driving) or led to low-level image discontinuities called salient regions (e.g. bright regions, edges). The time the eyes remain in a given region also depends on its visual and semantic properties. 

The experience of a complete and integrated visual world is thus based on an abstract representation that covers general information about the scene combined with perceptual information arisen from fixations. By examining eye movements, it could be possible to infer the underlying factors affecting fixations or task at hand, even to interpret observer thoughts \cite{defendingYarbus}. 

This is the purpose of our model in Chapter \ref{ch:atom}, which introduces an intermediate level between feature extraction and visual attention computation stages based on the information drawn from fixations. This level consists of latent sub-tasks that can be used to determine why some locations are more conspicuous than others. Thus, rather than directly learn a predictor of human attention over low-level visual features, our method provides a hierarchical interpretation of visual attention, advantageous for further comprehensive analysis.

The experiments conducted by Yarbus have motivated researchers to assess the possibilities of eye tracking for assistance in real applications such as industry control \cite{sharma2016eye}, health-care \cite{hermens2013eye} and video surveillance \cite{howard2011task}. Experts in these applications have to process a large amount of visual information at the same time, which implies a high cognitive effort that might be reduced by modeling fixations behavior along time. Indeed, it has been observed that there is a strong correlation between fixation patterns of different viewers performing the same task, specially during an important or suspicious event \cite{howard2013suspiciousness,sharma2016eye}.

The latter is the ultimate objective of our system in Chapter \ref{ch:anomaly_detection}, which is trained to model a temporal attention response arisen from fixations dispersion across viewers. 

\section{Computational modeling of visual attention}\label{sec:computational_va}
%%Evolution of computational visual attention models
%%(See article with scheme + State-of-the-art in visual attention)
\begin{figure*}
\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red] 
 % use timeline header]
 % timeline title={The title}]
1985 & Koch and Ullman \cite{koch_shifts} \endlr
1998 & Itti et al. \cite{Itti:1998:MSV:297843.297870} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Green]
2003 & Sprage and Ballard \cite{sprague2003eye} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=YellowOrange]
\ \ \ \ \ \ \ \ & Torralba \cite{Torralba:03} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Green]
2005 & Bruce and Tsotsos (\acs{AIM}) \cite{BruceT05} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Gray]
\ \ \ \ \ \ \ \ & Navalpakkam and Itti \cite{1641004} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=YellowOrange]
\ \ \ \ \ \ \ \ & Itti and Baldi \cite{Itti_Baldi06nips} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red] 
2006 & Harel et al. (\acs{GBVS}) \cite{Harel07graph-basedvisual} \endlr
2007 & Hou and Zhang \cite{HouZhang} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Gray]
\ \ \ \ \ \ \ \ & Peters and Itti \cite{peters2007beyond} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Purple]
2008 & Zhang et al. (\acs{SUN}) \cite{doi:10.1167/8.7.32} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red] 
2009 & Hou and Zhang (\acs{ICL}) \cite{hou2009dynamic} \endlr
\ \ \ \ \ \ \ \ & Seo and Milanfar (\acs{SDSR}) \cite{SeoMilanfar} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Green]
\ \ \ \ \ \ \ \ & Judd et al. \cite{judd2009learning} \endlr
\end{vtimeline} 

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Purple]
\ \ \ \ \ \ \ \ & Zhang et al. (Dynamic \acs{SUN}) \cite{zhang2009sunday} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red] 
2010 & Rahtu et al. (ESA-D) \cite{Rahtu2010} \endlr
\ \ \ \ \ \ \ \ & Guo and Zhang (\acs{PQFT}) \cite{5223506} \endlr
\ \ \ \ \ \ \ \ & Goferman et al. \cite{Goferman} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Green]
\ \ \ \ \ \ \ \ & Elazary and Itti \cite{Elazary20101338} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red] 
2011 & López-García et al. (\acs{WMAP}) \cite{lopez2011scene} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Purple]
\ \ \ \ \ \ \ \ & Li et al. \cite{5733396} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red] 
2012 & García-Díaz et al. (\acs{AWS}) \cite{GallegaSaliency2012} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=NavyBlue]
2014 & Vig et al. \cite{vig2014deep} \endlr
\ \ \ \ \ \ \ \ & Kümmerer et al. (DeepGaze I) \cite{kummerer2014deepgaze1} \endlr
2015 & Huang et al. (SALICON) \cite{huang2015salicon} \endlr
2016 & Kümmerer et al. (DeepGaze II) \cite{kummerer2016deepgaze2} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Sepia]
\ \ \ \ \ \ \ \ & Li et al. (DCL) \cite{DeepSaliencyObject} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Red]
2017 & Leborán et al.(\acs{AWS-D}) \cite{GallegaSaliency} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=NavyBlue]
\ \ \ \ \ \ \ \ & Kruthiventi et al. (DeepFix) \cite{kruthiventi2017deepfix} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Rhodamine]
\ \ \ \ \ \ \ \ & Jiang et al. \cite{ledov} \endlr
2018 & Bak et al. \cite{bak2018spatio} \endlr
\ \ \ \ \ \ \ \ & Wang et al. \cite{dhf1k} \endlr
\ \ \ \ \ \ \ \ & Cornia et al. (\acs{SAM}) \cite{lstm2018cornia} \endlr
\end{vtimeline}

\begin{vtimeline}[description={text width=10cm}, 
 row sep=1ex, timeline color=Sepia]
\ \ \ \ \ \ \ \ & Wang et al. \cite{wang2018video} \endlr
\end{vtimeline}

\caption*{\tikz\draw[fill=Red] (0,0) circle (.5ex); \acs{BU} models\hspace{5mm} \tikz\draw[fill=Green] (0,0) circle (.5ex); \acs{TD} models\hspace{5mm} \tikz\draw[fill=Gray] (0,0) circle (.5ex); \acs{BU}+\acs{TD} models\hspace{5mm} \tikz\draw[fill=YellowOrange] (0,0) circle (.5ex); Bayesian \acs{BU} models\\ \tikz\draw[fill=Purple] (0,0) circle (.5ex); Bayesian \acs{TD} models\hspace{5mm} \tikz\draw[fill=NavyBlue] (0,0) circle (.5ex); Deep static models\hspace{5mm} \tikz\draw[fill=Rhodamine] (0,0) circle (.5ex); Deep dynamic models\hspace{5mm}\\ \tikz\draw[fill=Sepia] (0,0) circle (.5ex); Deep salient object detection models \hspace{5mm}}
\caption{Chronological timeline of the visual attention models in the \emph{state-of-the-art} reviewed in this thesis.}\label{fig:saliency_timeline}
\end{figure*}

So far, we have reviewed how vision and visual attention work in humans. Similarly, vision in camera systems depends on the interaction among light, surfaces that reflect light, and a visual system that can detect light. Furthermore, both human eyes and cameras share certain physical similarities, and the same optical function: they gather light reflected from objects in order to obtain a sharply-focused image. 

However, while humans acquire knowledge about their surroundings, being able to respond to a given situation, cameras have no perceptual capabilities, so they can not interpret their recordings at all. As cameras are not able to deal with attention processes, computer vision researchers have developed automatic systems which efficiently determine the most appealing regions from images or videos, by means of \acfp{VAM}.

This section provides a review of some of the existing visual attention algorithms in the \emph{state-of-the-art}, referring both to \acs{BU} and \acs{TD} methods. We will specially focus on those that are closely related to our approaches, and also on promising deep learning-based architectures. All the models explained in the following paragraphs are summarized in Figure \ref{fig:saliency_timeline} in chronological order. For further information, a exceptional detailed survey on visual attention modeling is presented by Borji et al. \cite{Borji:2013:SVA:2412386.2412937}.

\subsection{Bottom-up versus top-down approaches}\label{sec:computational_bu_td} 
On the basis of Treisman and Gelade's \acs{FIT} \cite{TreismanGelade80}, Koch and Ullman \cite{koch_shifts} presented in 1985 a design to combine early vision features, and defined the concept of \acs{SM}, which was subsequently mentioned in Wolfe's \acs{GSM} as a mechanism to model local visual attention driven by the set of visual stimuli in the scene. 

The first implementation and verification of a \acs{BU} model, performed by Itti et al. \cite{Itti:1998:MSV:297843.297870}, and incorporating color, intensity and orientation features, would nevertheless come more than ten years later. After that, Harel et al. \cite{Harel07graph-basedvisual} proposed a saliency algorithm based on graphs, which extracted the same features at different scales. These two representations are the most frequently employed in the literature due to their good performance in a variety of applications \cite{yubing2011spatiotemporal, wang2013airport, ferfer2017exploiting}.

The great majority of visual attention models developed are \acs{BU} approaches, as the ones explained below. It is also surprising the lack of use and modeling of spatio-temporal and high-level features to address visual attention in real scenarios or videos, although almost half of the methods found in the literature are dynamic ones.

% Bottom-up
% - Characteristics of the visual scene
% - Salient object detection
\begin{itemize}
\item \emph{Itti et al., 1998} \cite{Itti:1998:MSV:297843.297870}: Related to \acs{FIT} \cite{TreismanGelade80} and in accordance with the biological architecture proposed by Koch and Ullman \cite{koch_shifts}, it is the first existing implementation of a spatial saliency model. It decomposes visual input into a set of topographic feature maps of color, intensity and orientation. The three conspicuity maps are normalized and summed constituting the \acs{SM}, whose maximum determines the most salient image region. 

Additionally, the authors propose a later stage to determine the order in which fixations may occur based on the \acs{SM} obtained. To this end, the \acs{SM} is modeled as a \acf{2D} layer of leaky integrate-and-fire neurons which feeds into a biologically-plausible \acf{WTA} neural network. Each \acs{SM} neuron excites its corresponding \acs{WTA} neuron, until the most salient ("the winner") fires. This causes the \acf{FOA} to be shifted to the location of the winner neuron. After this, all neurons are reset, and an \acf{IOR} mechanism is activated, which either allows the next most salient area to become the following winner or prevents the \acs{FOA} from shortly reaching an attended region. 

\item \emph{Harel et al., 2006} \cite{Harel07graph-basedvisual}: This spatial \acs{BU} saliency algorithm based on graphs extracts the same multi-scale features than Itti et. al \cite{Itti:1998:MSV:297843.297870}. \acf{GBVS} then computes a fully connected graph over all feature map grid locations, by assigning weights between each two nodes that are proportional to the similarity of feature values and their spatial distance. The obtained graphs proceed as Markov chains that define an equivalence relation either between nodes and states or edge weights and transition probabilities. Their associated equilibrium distribution results in activation maps, whose combination gives rise eventually to the \acs{SM}.

\item \emph{Hou and Zhang, 2007} \cite{HouZhang}: Hou and Zhang first proposed a spectral residual saliency model for static images. On the basis that statistical singularities in the spectrum may determine the anomalous regions of a given image, they derive its amplitude and phase. Then, they compute the log-spectrum of the down-sampled image. After that, the spectral residual is obtained by multiplying by a local average filter, and subtracting the result from itself. Finally, the \acs{SM} is built in the spatial domain by using the \acf{IFT} and squaring the value of each point to indicate the estimation error. 

\item \emph{Hou and Zhang, 2009} \cite{hou2009dynamic}: Their next approach to saliency, called \acf{ICL}, is a principle that tries to maximize the overall entropy gain of a given set of sample visual features, now both in dynamic and static settings. Salient cues are those unexpected feature values that produce an entropy gain in the perception state. Therefore, features with large coding length increments will allow to reach attention selectivity. 
 
\item \emph{Seo and Milanfar, 2009} \cite{SeoMilanfar}: The \acf{SDSR} spatio-temporal framework computes local regression kernel descriptors given an image or video. Each pixel or voxel in the \acs{SM} indicates the statistical likelihood of saliency of a feature matrix given its surrounding feature matrices. According to the authors, the use of \acf{LSK} as features instead of conventional filter responses captures the underlying local structure of the data, even in the presence of significant distortions. % Se puede ampliar la explicacion, ver paper Master

\item \emph{Rahtu et al., 2010} \cite{Rahtu2010}: This spatio-temporal method, named ESA-D, proposes a combination of a statistical saliency measure based on contrasts in illumination, color and motion, together with a \acf{CRF} model for salient object detection. The motivation of the authors to determine the most appealing areas by minimizing an energy function derived from a \acs{CRF} is that saliency estimation objective is usually to achieve an object-level segmentation instead of a pixel-level one. 

\item \emph{Guo and Zhang, 2010} \cite{5223506}: The authors propose the \acf{PQFT} method, which carries out a quaternion representation of video frames by means of intensity, color and motion features. Moreover, they also implement a foveation approach based on a wavelet multiresolution representation, with the purpose of improving video compression efficiency.  

\item \emph{Goferman et al., 2010} \cite{Goferman}: This context-aware saliency model takes into account four psychological principles of human attention: 1) local low-level features, such as color and contrast; 2) global factors, which stand out features that differ from the norm; 3) visual organization rules related to forms and 4) a high-level face detector.    

\item \emph{López-García et al., 2011} \cite{lopez2011scene}: The authors propose the \acf{WMAP} measure as a spatial visual attention estimator with the purpose of significantly accelerating a scene recognition task, preserving its performance. The approach considers both efficient coding, in order to reduce the redundancy of the input data, and the detection of important attributes of the image via local edge phase and energy.

\item \emph{García-Díaz et al., 2012} \cite{GallegaSaliency2012}: The \acf{AWS} model provides a measure of saliency by considering the local energy variability in the $Lab$ color space. First, a Gabor bank of filters is applied to the luminance channel $L$, extracting several multioriented multiresolution features. On the other hand, a multiscale decomposition of the $a$ and $b$ color components is computed. Finally, a \acf{PCA} is performed over all these low-level representations in order to decorrelate them, obtaining the local measure of variability that underlies the \acs{SM}. 

\item \emph{Leborán et al., 2017} \cite{GallegaSaliency}: This approach, called \acf{AWS-D}, is an extension of the \acs{AWS} \cite{GallegaSaliency2012} explained above that computes either static or dynamic saliency maps. The hypothesis of the authors is that saliency has a strong relationship with the variability of the local energy measured over a statistically decorrelated and normalized space. Thus, in order to estimate saliency, the model looks for the space-time points with maximum variability in the distribution of the local energy across spatio-temporal scales and orientations. In contrast to other spatio-temporal methods, it does not rely on information derived from a explicit background model or the estimation of optical flow to compute motion features. 

\end{itemize}

% Top-down
% - + eye movements 
In contrast, \acs{TD} architectures are still scarce and very often tailored to well-defined scenarios. In such cases, the evaluation of the whole scheme is performed regardless of the capability of the guidance tool. What is more, most \acs{TD} approaches guide attention towards specific targets by modulating gains associated with low-level stimuli.

\begin{itemize}
\item \emph{Sprague and Ballard, 2003} \cite{sprague2003eye}: They present a reinforcement learning method that combines action selection and visual perception in a sidewalk navigation task. 

\item \emph{Bruce and Tsotsos, 2005} \cite{BruceT05}: The \acf{AIM} model proposed computes a \acs{VAM} based on the Shannon's self-information measure. At each image region, saliency is the information that the region conveys with respect to its surroundings. The information of the visual feature is inversely proportional to the likelihood of observing it. Consequently, to calculate this feature, the \acf{PDF} has to be estimated. Moreover, in order to reduce the dimensionality of the problem, an \acf{ICA} is performed. Thus, given a local image region, the probability of observing the $RGB$ values is estimated via the product of the likelihood of the components associated to that region.      

\item \emph{Judd et al., 2009} \cite{judd2009learning}: The model is based on a linear \acf{SVM}, taking some image features and human fixations to define salient locations. 

\item \emph{Elazary and Itti, 2010} \cite{Elazary20101338}: They propose a more flexible \acs{TD} model that can concurrently select the best features to guide attention and adjust the width of feature detectors. 

\end{itemize}

Finally, although suggested by the prevalent studies about attention \cite{Yarbus1967, wolfe1994guided}, just a few works propose hybrid models incorporating \acs{BU} and \acs{TD} factors. 

\begin{itemize}
\item \emph{Navalpakkam and Itti, 2005} \cite{1641004}: The model optimizes the integration of \acs{BU} cues for target detection by maximizing the signal-to-noise ratio of the target versus background. 

\item \emph{Peters and Itti, 2007} \cite{peters2007beyond}: This model computes a task-dependent map based on the scene gist and the eye fixations gathered from a video games scenario. \acs{BU} and \acs{TD} integration is simply conducted as a multiplication of both components. 
\end{itemize}

\subsection{Bayesian models}\label{computational_bayesian} 
Since our model proposed in Chapter \ref{ch:atom} is based on a Bayesian formulation of visual attention, this section briefly introduces some Bayesian or probabilistic approaches found in the \emph{state-of-the-art}. 

On the one hand, probabilistic \acs{BU} algorithms make use of Bayes' rule to combine the features observed with prior constrains:

\begin{itemize}
\item \emph{Torralba, 2003} \cite{Torralba:03}: The author presents a Bayesian approach for visual search tasks. \acs{BU} saliency stands on a global feature based on the scene gist, which provides a shortcut to detect the presence or absence of objects in an image before exploring it.

\item \emph{Itti and Baldi, 2005} \cite{Itti_Baldi06nips}: They propose a probabilistic framework for modeling saliency as ``surprise'' by computing the \acs{KL} divergence between the posterior and prior beliefs about image features, either in space or time domains. 
\end{itemize}

On the other hand, Bayesian \acs{TD} models are characterized by their capacity to learn from data, taking advantage of data statistics to model the underlying attention process and allowing to obtain interpretable relationships between data and visual fixations:

\begin{itemize}
\item \emph{Zhang et al., 2008} \cite{doi:10.1167/8.7.32}: This framework understands saliency as the point-wise mutual information between \acs{BU} local features and \acs{TD} search target features. The model, known as \acf{SUN}, tries to reproduce the visual experience acquired by an organism. To achieve this, it defines visual saliency as the probability of a searched target at every point in the visual field given the features observed. Using Bayes' rule, and assuming that feature and location are independent, the self-information is taken as definition of \acs{BU} saliency: the rarer a feature is, the more it will attract our attention. Given this definition, features are calculated as responses of biologically plausible linear filters, such as \acf{DoG} and Gabor filters, as same as in \cite{Itti:1998:MSV:297843.297870}, and also as the responses to filters learned from natural images, using \acs{ICA}. 

After this first approach, the model was extended to temporally dynamic scenes in \cite{zhang2009sunday}, characterizing the video statistics around each pixel using a bank of spatio-temporal filters with separable space-time components.

\item \emph{Li et al., 2011} \cite{5733396}: They provide a multi-task learning approximation for visual attention in video, where different ranking functions for fusing \acs{BU} and \acs{TD} maps are learned depending on the scene content.  
\end{itemize}

%% DEEP LEARNING
\subsection{Deep Neural Networks}\label{sec:computational_cnn} 
\acfp{CNN} \cite{lecun1989backpropagation, simard2003best}, the current dominant paradigm for many supervised tasks in computer vision, have also been applied to model visual attention achieving promising results, especially in the still image domain. Furthermore, either for \acsp{SM} refinement based on attention modules or visual attention estimation in video, researchers have recently drawn on recurrent \acf{LSTM}-based networks \cite{hochreiter1997long}.

\acsp{DNN} involve training end-to-end models according to a loss function, using a database of images or videos annotated with \acs{GT} fixations. They unify feature extraction, fusion and saliency prediction into a single structure. This usually improves the system performance at the expense of making the analysis of these stages more challenging, mainly due to the abstract nature of representations at the deepest layers of these strategies.

Among the first attempts to rely on deep learning for static saliency estimation, the following ones deserve our analysis:

\begin{itemize}
\item \emph{Vig et al., 2014} \cite{vig2014deep}: It constitutes one of the first approaches that makes use of \acs{CONV} layers for saliency prediction, training a softmax classifier on top of them, so that \acsp{SM} are formulated as generalized Bernoulli distributions.

\item \emph{Kümmerer et al., 2014} \cite{kummerer2014deepgaze1}, \emph{2016} \cite{kummerer2016deepgaze2}: First, in 2014, the authors present Deep Gaze I, which builds \acsp{SM} by using the object recognition model of Krizhevsky et al. \cite{krizhevsky2012imagenet} and a prior distribution to model the central fixation bias \cite{kummerer2014deepgaze1}. Further on, in 2016, Deep Gaze II \cite{kummerer2016deepgaze2} applies transfer learning to saliency prediction by fine-tuning a few layers on top of the features from a VGG network \cite{vgg2014}, also for object recognition.
 
\item \emph{Huang et al., 2015} \cite{huang2015salicon}: The SALICON fine- and coarse-scale model evaluates the use of four commonly-known differentiable saliency metrics as the objective function of a simple \acs{CNN} architecture, providing image \acsp{SM} which integrate information at different scales.  Furthermore, the authors introduce a large-scale image dataset \cite{jiang2015salicon} for training new models, annotated by means of a mouse-tracking procedure, which seemed to correlate well with human fixations.

\item \emph{Kruthiventi et al., 2017} \cite{kruthiventi2017deepfix}: The authors present DeepFix, a fully \acs{CNN} built on top of a VGG network \cite{vgg2014} for hierarchically modeling the \acs{BU} mechanism of visual attention. The network captures semantics at multiple scales and information derived from the global context, and also models center-bias effect in human attention. 

\item \emph{Cornia et al., 2018} \cite{lstm2018cornia}: \acs{SAM} model is able to predict accurate \acsp{SM} by incorporating a neural attentive mechanism based on convolutional \acsp{LSTM} \cite{xingjian2015convolutional}. Given a \acs{SM}, the method refines it by iteratively focusing on the most prominent regions, and also considering the center bias existing in human fixations by learning a set of prior Gaussian maps. 
\end{itemize}

Despite the outstanding performance achieved by these approaches, they still miss some key elements \cite{DBLP:conf/eccv/BylinskiiRBOTD16}, mostly related to mis-detections of people, actions and text, and the relative importance assigned to them when they take place simultaneously. 

It should also be pointed out that only a few works have drawn on deep learning to tackle the estimation of visual attention in videos:

\begin{itemize}
\item \emph{Jiang et al., 2017} \cite{ledov}: Together with a large-scale eye-tracking database of generic videos, the authors propose a \acs{CNN} to learn spatio-temporal features based on object motion, and also a two-layer convolutional \acs{LSTM} network to smooth the transition between \acsp{SM} of consecutive frames.

\item \emph{Bak et al., 2018} \cite{bak2018spatio}: The authors study the use of dynamic models for saliency prediction in videos, providing several single and two-stream \acsp{CNN} and evaluating different fusion mechanisms to combine spatial and temporal information. They demonstrate the importance of considering inherent motion information, by training models on estimated optical flow. % \cite{DBLP:journals/corr/BakEE16}

\item \emph{Wang et al., 2018} \cite{dhf1k}: Similarly to \cite{ledov}, the authors share a new large-scale database of videos with fixations, organized by their categories, and then present a \acs{CNN}-\acs{LSTM} architecture with an attention mechanism. The \acs{CNN} encodes the static saliency information, which allows the \acs{LSTM} to learn temporal saliency representations for successive video frames.
\end{itemize}

Finally, \acsp{CNN} have also been applied to a particular type of saliency, closely related to the object detection task, both in images or videos. These models provide a map of objectness, measuring the probability that each image location belongs to an object. Nevertheless, these networks are often trained on databases with \acs{GT} object segmentation masks instead of fixations.

\begin{itemize}
\item \emph{Li et al., 2016} \cite{DeepSaliencyObject}: The authors present an end-to-end deep contrast network for salient object detection. The network consists of a pixel-level \acs{FC} stream, which generates a \acs{SM} with pixel-level accuracy, and a segment-wise spatial pooling stream, which improves the modeling of saliency discontinuities along object boundaries. Moreover, at the end of these two streams, a \acs{CRF} model can be applied to improve the spatial coherence and contour localization. 
 
\item \emph{Wang et al., 2018} \cite{wang2018video}: They provide a efficient framework for object detection in videos that captures spatial and temporal saliency information via a short-term analysis consisting of learning from adjacent frame pairs, without the need to compute optical flow.
\end{itemize}

The reader is also referred to a recently released survey by Ali Borji about deep learning-based models for saliency prediction in images and videos \cite{borji2018saliency}, where he also discusses emerging applications of these architectures and which aspects should be considered in order to improve them.

\subsection{Applications}\label{sec:computational_applications}
Computer vision techniques have nowadays to deal with millions and millions of available data, just as the \acs{HVS} does. This is probably the prime reason why the effort in developing computational systems to accomplish the selective task carried out by visual attention has increased during the last few years. 

We can highlight two main purposes for visual attention modeling \cite{borji2018saliency}:

\begin{itemize}
\item The first, related to our contributions in Chapters \ref{ch:atom} and \ref{ch:atom_experiments}, is to understand \emph{how} visual attention works in humans, trying to describe the behavioral and neural processes that it involves. 

\item The second is to predict \emph{where} people look, in order to address traditional image and video applications, such as object \cite{ivanNUS,IEEEVideoObjectRecognition} and action \cite{IEEEVideoActionRecognition, WangCNNAction} recognition, video summarization \cite{Ma:2002:UAM:641007.641116}, patient diagnosis \cite{Chaabouni2017} or image quality assessment \cite{IEEEVideoImageQuality}, in broader and more complex scenarios, while providing efficient solutions and better performances. In line with the second objective, our contributions in Chapters \ref{ch:anomaly_detection} and \ref{ch:surveillance_experiments} pursue to facilitate the task of a \acs{CCTV} operator in a video surveillance scenario, by means of a deep architecture that models attention in the temporal domain. 
\end{itemize}

%\subsubsection*{Video surveillance}
%In line with the second objective, our contributions in Chapters \ref{ch:anomaly_detection} and \ref{ch:surveillance_experiments} pursue to facilitate the task of a \acs{CCTV} operator in a video surveillance scenario, by means of a deep architecture that models attention in the temporal domain. 
%
%A video surveillance scenario involves... COMPLETE

%Anomaly detection
%-Souad application
%-Ivan application (egocentric video)
%-studying car driving-related attentional mechanisms \cite{DBLP:journals/corr/PalazziSCAC16} and recognizing human activities \cite{WangCNNAction}.
%-surveillance,automatic target detection,navigational aids, robotic control

%\subsection{Models for eyes and gaze}\label{sec:eye_tracking_va}
%Eye tracking devices

%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/Chapter02demo.tex <==
%*****************************************
\chapter{Examples Demo}\label{ch:examples_demo}
%*****************************************
%\setcounter{figure}{10}
% \NoCaseChange{Homo Sapiens}
Ei choro aeterno antiopam mea, labitur bonorum pri no
\citeauthor{taleb:2012} \citep{taleb:2012}. His no decore
nemore graecis. 
suavitate interpretaris eu, vix eu libris efficiantur.
 Some interesting books in order to get a multi-page bibliography: \cite{ferriss:2016,greenwald:2014,adams:2013,pausch:2008,aurelius:2002,adams:1996,trump:1987,feynman:1985,cialdini:1984,seneca,orwell:1949,taleb:2010,munger:2008,postman:2005,frankl:1959} %\nocite{*}


\section{A New Section}
Examples: \textit{Italics}, \spacedallcaps{All Caps}, \textsc{Small
Caps}, \spacedlowsmallcaps{Low Small Caps}.

Acronym testing: \ac{UML} -- \acs{UML} -- \acf{UML} -- \acp{UML}


\section{Another Section in This Chapter} % 
\begin{description}
    \item[Description-Label Test:] Illo secundo continentes sia il, sia.
    \item[basate americano sia:] Lo vista ample programma pro, uno
    europee addresses ma.
\end{description}

\subsubsection{A Subsubsection}
\begin{aenumerate}
    \item Enumeration with small caps (alpha)
    \item Second item
\end{aenumerate}

\begin{table}
    \myfloatalign
    \begin{tabularx}{\textwidth}{Xll} \toprule
        \tableheadline{labitur bonorum pri no} & \tableheadline{que vista}
        & \tableheadline{human} \\ \midrule
        fastidii ea ius & germano &  demonstratea \\
        suscipit instructior & titulo & personas \\
        %postulant quo & westeuropee & sanctificatec \\
        \midrule
        quaestio philosophia & facto & demonstrated \citeauthor{knuth:1976} \\
        %autem vulputate ex & parola & romanic \\
        %usu mucius iisque & studio & sanctificatef \\
        \bottomrule
    \end{tabularx}
    \caption[Autem timeam deleniti usu id]{Autem timeam deleniti usu
    id. \citeauthor{knuth:1976}}  \label{tab:example}
\end{table}

\enlargethispage{2cm}
\subsection{Linguistic Registrate}
Lo sed apprende instruite. Que altere responder su, pan ma, \ie, signo
studio. \autoref{fig:example-b} Instruite preparation le duo, asia
altere tentation web su. Via unic facto rapide de, iste questiones
methodicamente o uno, nos al.

\begin{figure}[bth]
    \myfloatalign
    \subfloat[Asia personas duo.]
    {\includegraphics[width=.45\linewidth]{gfx/example_1}} \quad
    \subfloat[Pan ma signo.]
    {\label{fig:example-b}%
        \includegraphics[width=.45\linewidth]{gfx/example_2}} \\
    \subfloat[Methodicamente o uno.]
    {\includegraphics[width=.45\linewidth]{gfx/example_3}} \quad
    \subfloat[Titulo debitas.]
    {\includegraphics[width=.45\linewidth]{gfx/example_4}}
    \caption[Tu duo titulo debitas latente]{Tu duo titulo debitas
    latente. \ac{DRY}}\label{fig:example}
\end{figure}


%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/Chapter03.tex <==
%************************************************
\chapter{An introduction to representation learning and its applications in Computer Vision}\label{ch:rlearning_cvision} 
\chaptermark{An intro to RL and its applications in CV}
%************************************************

%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/Chapter03demo.tex <==
%************************************************
\chapter{Math Test Chapter Demo}\label{ch:mathtest_demo} % $\mathbb{ZNR}$
%************************************************
Ei choro aeterno antiopam mea, labitur bonorum pri no. His no decore
nemore graecis. In eos meis nominavi, liber soluta vim cu. Sea commune
suavitate interpretaris eu, vix eu libris efficiantur.

\section{Some Formulas}
The description of ionisation fluctuations is
characterised by the significance parameter $\kappa$, which is
proportional to the ratio of mean energy loss to the maximum allowed
energy transfer in a single collision with an atomic electron:
\graffito{You might get unexpected results using math in chapter or
section heads. Consider the \texttt{pdfspacing} option.}
\begin{equation}
\kappa =\frac{\xi}{E_{\textrm{max}}} %\mathbb{ZNR}
\end{equation}
$E_{\textrm{max}}$ is the maximum transferable energy in a single
collision with an atomic electron.
\[
E_{\textrm{max}} =\frac{2 m_{\textrm{e}} \beta^2\gamma^2 }{1 +
2\gamma m_{\textrm{e}}/m_{\textrm{x}} + \left ( m_{\textrm{e}}
/m_{\textrm{x}}\right)^2}\ ,
\]
where $\gamma = E/m_{\textrm{x}}$, $E$ is energy and
$m_{\textrm{x}}$ the mass of the incident particle,
$\beta^2 = 1 - 1/\gamma^2$ and $m_{\textrm{e}}$ is the electron mass.
$\xi$ comes from the Rutherford scattering cross section
and is defined as:
\begin{eqnarray*} \xi  = \frac{2\pi z^2 e^4 N_{\textrm{Av}} Z \rho
\delta x}{m_{\textrm{e}} \beta^2 c^2 A} =  153.4 \frac{z^2}{\beta^2}
\frac{Z}{A}
  \rho \delta x \quad\textrm{keV},
\end{eqnarray*}
where

\begin{tabular}{ll}
$z$          & charge of the incident particle \\
$N_{\textrm{Av}}$     & Avogadro's number \\
$Z$          & atomic number of the material \\
$A$          & atomic weight of the material \\
$\rho$       & density \\
$ \delta x$  & thickness of the material \\
\end{tabular}

$\kappa$ measures the contribution of the collisions with energy
transfer close to $E_{\textrm{max}}$.  For a given absorber, $\kappa$
tends
towards large values if $\delta x$ is large and/or if $\beta$ is
small.  Likewise, $\kappa$ tends towards zero if $\delta x $ is small
and/or if $\beta$ approaches $1$.

The value of $\kappa$ distinguishes two regimes which occur in the
description of ionisation fluctuations:

\begin{enumerate}
\item A large number of collisions involving the loss of all or most
    of the incident particle energy during the traversal of an absorber.

    As the total energy transfer is composed of a multitude of small
    energy losses.
    
\item Particles traversing thin counters and incident electrons under
    any conditions.

    The relevant inequalities and distributions are $ 0.01 < \kappa < 10
    $,
    Vavilov distribution, and $\kappa < 0.01 $, Landau distribution.
\end{enumerate}


\section{Various Mathematical Examples}
If $n > 2$, the identity
\[
    t[u_1,\dots,u_n] = t\bigl[t[u_1,\dots,u_{n_1}], t[u_2,\dots,u_n]
    \bigr]
\]
defines $t[u_1,\dots,u_n]$ recursively, and it can be shown that the
alternative definition
\[
    t[u_1,\dots,u_n] = t\bigl[t[u_1,u_2],\dots,t[u_{n-1},u_n]\bigr]
\]
gives the same result.

%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/Chapter0C.tex <==
%********************************************************************
% Appendix
%*******************************************************
% If problems with the headers: get headings in appendix etc. right
%\markboth{\spacedlowsmallcaps{Appendix}}{\spacedlowsmallcaps{Appendix}}
\chapter{Spanish Introduction and Conclusions}\label{ch:spanish_info}

\section{Introducción}
\subsection{Motivación}
\subsection{Objetivos}
\subsection{Estructura de la tesis}

\section{Conclusiones y líneas futuras de investigación}
\subsection{Conclusiones}
\subsection{Líneas futuras de investigación}

==> FrontBackmatter/Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}
Put your declaration here.
\bigskip

\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{5cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}


==> FrontBackmatter/DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip

    \begingroup
        \color{RoyalBlue}\spacedallcaps{\myTitle}
    \endgroup
\end{center}


==> FrontBackmatter/Titleback.tex <==
\thispagestyle{empty}

% \hfill

% \vfill

% \noindent\myName: \textit{\myTitle,} \mySubtitle, %\myDegree,
% \textcopyright\ \myTime

%\bigskip
%
%\noindent\spacedlowsmallcaps{Supervisors}: \\
%\myProf \\
%\myOtherProf \\
%\mySupervisor
%
%\medskip
%
%\noindent\spacedlowsmallcaps{Location}: \\
%\myLocation
%
%\medskip
%
%\noindent\spacedlowsmallcaps{Time Frame}: \\
%\myTime


==> FrontBackmatter/Tribunal.tex <==
\thispagestyle{empty}

\noindent Tesis doctoral: \\
\noindent \spacedlowsmallcaps{\myTitle} \\

\noindent Autor: \\
\noindent \spacedlowsmallcaps{\myName} \\

\noindent Directores: \\
\noindent \spacedlowsmallcaps{\myProf} \\
\noindent \spacedlowsmallcaps{\myOtherProf} \\

\vspace{2cm}

El tribunal nombrado para juzgar la tesis doctoral arriba citada, compuesto por los doctores: \\

\noindent Presidente: \\

\noindent Secretario: \\

\noindent Vocal: \\

\noindent acuerda otorgarle la calificación de: \\

Leganés, a ... \\

